A Mobile Impurity in the Kitaev Chain: Phase Diagram and Signatures of Topology

We study the physics of a mobile impurity immersed in a $1d$ topological superconductor. We discuss the system's phase diagram obtained with exact diagonalization. We argue that the character of the transition from a weak to strong coupling regime depends on the phase of the host superconductor. A smooth crossover between a weakly coupled polaron and a molecular state is observed in the topological phase. In contrast, the impurity undergoes a sharp phase transition in a topologically trivial background.

==> zapas/zapas.tex <==
Also, using standard Jordan-Wigner transformation and setting $t_c = \Delta$ the Kitaev chain Eq.\eqref{kit} maps on the spin-$\frac{1}{2}$ chain:

\begin{equation}\label{kit_orig_spin}

H_\text{Kit} = -\sum_{i=1}^N \left( 4t_c S^y_i S^y_{i+1} + \mu S^z_i\right) - \frac{\mu N}{2}, 

\end{equation}

where $S^\gamma_i$ are the Pauli spin operators with $\comm{S^\alpha_i}{S^\beta_j} = i\delta_{ij} \varepsilon_{\alpha\beta\gamma}S^\gamma_i$.




While the free part of the Hamiltonian remains unexcited, we can introduce a basis that includes the impurity on the $m$-th site and accounts for the creation of excitations and the excitation part can be written as
\begin{equation}
    h_\text{ex} = \begin{pmatrix}
        -2t_c &0 &0 &U \\
       0 &0 &U &0 \\
       0 &U &0 &0 \\
       U &0 &0 &2t_c
    \end{pmatrix}.
\end{equation}
\textcolor{red}{If $U = 0$ the minimal eigenvalue of $h_{\text{ex}}$ is $\epsilon_\text{min} = -2t_c$ with the vector $\ket{\psi(U=0)} = \ket{0,0}$, so the topological ground state $\ket{\text{top}}$ is recovered. As $U\rightarrow +\infty$ there is a double degeneracy that leads to the $\expval{h_\text{ex}}_{U\rightarrow+\infty} = 0$. Also, the magnetization $M_z$ is changing smoothly form $0$ to $-\frac{1}{2}$ (FIG.\ref{fig:bloch}: Red). Therefore, as $U$ increases the chain will opened and one should expect two unpaired Majorana fermions to be localized near the impurity.}



{\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{maj_free.jpg}
    \caption{Maforana correlation function for the closed Kitaev chain with $t_c=\Delta = 1, N=8$. The topological phase is in the range $\mu\in [-2,-2]$, trivial phase is everywhere outside this range.}
    \label{fig:maj_free}
\end{figure}
